Uncertainty Quantification in Synthetic Controls with Staggered Treatment Adoption

We propose principled prediction intervals to quantify the uncertainty of a large class of synthetic control predictions (or estimators) in settings with staggered treatment adoption, offering precise non-asymptotic coverage probability guarantees. From a methodological perspective, we provide a detailed discussion of different causal quantities to be predicted, which we call causal predictands, allowing for multiple treated units with treatment adoption at possibly different points in time. From a theoretical perspective, our uncertainty quantification methods improve on prior literature by (i) covering a large class of causal predictands in staggered adoption settings, (ii) allowing for synthetic control methods with possibly nonlinear constraints, (iii) proposing scalable robust conic optimization methods and principled data-driven tuning parameter selection, and (iv) offering valid uniform inference across post-treatment periods. We illustrate our methodology with an empirical application studying the effects of economic liberalization on real GDP per capita for Sub-Saharan African countries. Companion software packages are provided in Python, R, and Stata.

==> tables/estValueRegularizationParams.tex <==
\begin{tabular}{lcccccc}
\toprule\toprule
   \textit{Treated Unit}   & $Q^{[i]}, M=1$ & $Q^{[i]}, M=2$& $\mathcal{T}_i$ & $|\mathcal{T}_i|$  \\
\midrule
Benin & 2.041 & 0.699 & 1963 - 1989 & 27 \\
Botswana & 2.119 & 0.771 & 1963 - 1978 & 16 \\
Cabo Verde & 0.877 & 0.5   & 1963 - 1990 & 28 \\
Cameroon & 2.336 & 0.786 & 1963 - 1992 & 30 \\
Gambia & 1.401 & 1.035 & 1963 - 1984 & 22 \\
Ghana & 0.858 & 0.972 & 1963 - 1984 & 22 \\
Guinea & 0.591 & 0.65  & 1963 - 1985 & 23 \\
Guinea-Bissau & 0.942 & 0.718 & 1963 - 1986 & 24 \\
Ivory Coast & 1.212 & 0.838 & 1963 - 1993 & 31 \\
Kenya & 0.959 & 0.569 & 1963 - 1992 & 30 \\
Mali  & 1.445 & 0.65  & 1963 - 1987 & 25 \\
Mauritius & 1.705 & 1.145 & 1963 - 1967 & 5 \\
Niger & 2.252 & 1.793 & 1963 - 1993 & 31 \\
South Africa & 1.169 & 0.5   & 1963 - 1990 & 28 \\
Uganda & 1.797 & 0.5   & 1963 - 1987 & 25 \\
Zambia & 2.554 & 0.5   & 1963 - 1992 & 30 \\
\bottomrule\bottomrule
\end{tabular}%

==> tables/includedCountries.tex <==
\begin{tabular}{lcclc}
\toprule\toprule
Angola & \multicolumn{1}{l}{$\infty$} &       & Lesotho & $\infty$ \\
Benin & 1990  &       & Madagascar & \multicolumn{1}{r}{1996} \\
Botswana & 1979  &       & Malawi & $\infty$ \\
Burkina Faso & 1998  &       & Mali  & \multicolumn{1}{r}{1988} \\
Burundi & 1999  &       & Mauritius & \multicolumn{1}{r}{1968} \\
Cabo Verde & 1991  &       & Mozambique & \multicolumn{1}{r}{1995} \\
Cameroon & 1993  &       & Niger & \multicolumn{1}{r}{1994} \\
Chad  & \multicolumn{1}{l}{$\infty$} &       & Nigeria & $\infty$ \\
Congo & \multicolumn{1}{l}{$\infty$} &       & Rwanda & $\infty$ \\
Ethiopia & 1996  &       & Senegal & $\infty$ \\
Gabon & \multicolumn{1}{l}{$\infty$} &       & Sierra Leone & $\infty$ \\
Gambia & 1985  &       & South Africa & \multicolumn{1}{r}{1991} \\
Ghana & 1985  &       & Tanzania & \multicolumn{1}{r}{1995} \\
Guinea & 1986  &       & Togo  & $\infty$ \\
Guinea-Bissau & 1987  &       & Uganda & \multicolumn{1}{r}{1988} \\
Ivory Coast & 1994  &       & Zambia & \multicolumn{1}{r}{1993} \\
Kenya & 1993  &       & Zimbabwe & $\infty$ \\
\bottomrule\bottomrule
\end{tabular}%


==> tables/notation.tex <==
\begin{tabular}{p{0.35\linewidth}  p{0.65\linewidth}}
    \toprule\toprule
    \multicolumn{1}{l}{\textbf{Quantity}} & \multicolumn{1}{l}{\textbf{Description}} \\
    \midrule
    $\tau_{ik}$ & time-specific unit-specific predictand\\
    $\tau_{i\cdot}$ & time-averaged unit-specific predictand\\
    $\tau_{\mathcal{Q}k}$ & time-specific unit-averaged predictand\\
    $\tau_{\cdot\cdot}$& time-averaged unit-averaged predictand\\
    $\mathcal{N}$ & set of never-treated units\\
    $\mathcal{E}$ & set of ever-treated units\\
    $\mathcal{W}^{[i]}$ or $\mathcal{W}$ & 
    constraint set imposed in SC construction \\
    $J_0$ & number of never-treated units\\
    $J_1$ & number of ever-treated units\\
    $Q$ & number of units in $\mathcal{Q}$\\
    $Y_{it}$ & real GDP per capita of country $i$ in year $t$\\
    $\bY_{\mathcal{N}t}$& a vector of outcomes of never-treated (donor) units\\
    $u_{it}$ & out-of-sample error in decomposition of $\hat{Y}_{it}$\\
    $\varrho_\ell^{[i]}$ & tuning parameter used to check if the $\ell$-th constraint is binding\\
    $\mathcal{M}_{\widehat{\bgamma}}^{[i]}$ or
    $\mathcal{M}_{\widehat{\bgamma}}$ & feasible set for SC weights deduced from optimization\\
    $\mathcal{M}_{\bG}^{[i]\star}$ or $\mathcal{M}_{\bG}^{\star}$&
    feasible set used for in-sample uncertainty quantification\\
    $\Delta^{[i]}$ or $\Delta$ & centered constraint set\\
    $\mathrm{dist}(\ba, \mathcal{A})$ & 
    distance between a point $\ba$ and a set $\mathcal{A}$, i.e., $\inf_{\bm{\lambda}\in\mathcal{A}}\|\ba-\bm{\lambda}\|$\\
    $\mathcal{A}_\varepsilon$ & $\varepsilon$-enlargement of $\mathcal{A}$, i.e., $\{\ba:\mathrm{dist}(\ba, \mathcal{A})\leq\varepsilon\}$\\
    $|\mathcal{A}|$ & number of elements in a set $\mathcal{A}$\\
    $\times_{i\in\mathcal{S}}\mathcal{A}_i$ & Cartesian product of sets $\mathcal{A}_i$'s for $i\in\mathcal{S}$\\
    $\|\cdot\|_1$, $\|\cdot\|_2$ & L1 and L2 vector norms\\
    $s_{\min}(\bA)$, $s_{\max}(\bA)$ & minimum and maximum singular values of a matrix $\bA$\\
    $(v_j: j\in\mathcal{A})$ & a vector consisting of all $v_j$'s with $j\in\mathcal{A}$\\
    $\otimes$ & Kronecker product \\
    subscripts $\tin$, $\tout$ & ``in-sample'', ``out-of-sample''\\
    superscript $[i]$ & indicate a quantity is related to a treated unit $i$\\
    lower bar, upper bar & ``lower bound'', ``upper bound''\\
    $\star$ & indicate a quantity is related to simulation
    \\\bottomrule\bottomrule
    \end{tabular} 


==> tables/piLengthReduction.tex <==
\begin{tabular}{ccccccccc}
\toprule
\toprule
$\mathcal{W}$ & \multicolumn{2}{c}{\textit{Ridge}} &       & \multicolumn{2}{c}{\textit{Simplex}} &       & \multicolumn{2}{c}{\textit{L1-L2}} \\
\cmidrule{2-3}\cmidrule{5-6}\cmidrule{8-9}\multicolumn{1}{l}{Predictand} & $M=1$ & $M=2$ &       & $M=1$ & $M=2$ &       & $M=1$ & $M=2$ \\
\midrule
\multicolumn{1}{l}{\textit{All treated units }} &       &       &       &       &       &       &       &  \\
\multirow{2}[0]{*}{$\tau_{ik}$, Figure 3(a)} & 41.98 & 55.05 &       & 59.68 & 60.63 &       & 60.08 & 60.38 \\
      & $[16.80;92.28]$ & $[33.15;80.68]$ &       & $[17.70;93.56]$ & $[36.61;92.64]$ &       & $[11.66;92.92]$ & $[37.44;92.97]$ \\
      &       &       &       &       &       &       &       &  \\
\multirow{3}[0]{*}{$\tau_{i\cdot}$, Figure 4(a)} & 42.78 & 56.54 &       & 61.32 & 61.13 &       & 60.41 & 60.17 \\
      &       &       &       &       &       &       &       &  \\
      & $[21.08;87.87]$ & $[35.36;73.31]$ &       & $[22.20;93.66]$ & $[40.56;81.27]$ &       & $[15.28;91.55]$ & $[42.20;81.02]$ \\
      &       &       &       &       &       &       &       &  \\
\multirow{2}[0]{*}{$\tau_{\cdot k}$, Figure 6(a)} & 94.21 & 94.09 &       & 94.49 & 94.12 &       & 95.03 & 94.33 \\
      & $[94.06;94.24]$ & $[94.04;94.16]$ &       & $[94.40;95]$ & $[94.07;94.25]$ &       & $[94.77;95.11]$ & $[94.3;94.41]$ \\
      &       &       &       &       &       &       &       &  \\
\multicolumn{1}{l}{\textit{Countries Liberalized Before 1987}} &       &       &       &       &       &       &       &  \\
\multirow{2}[0]{*}{$\tau_{\mathcal{Q}_1 k}$, Figure 5(a)} & 76.65 & 78.91 &       & 78.04 & 78.04 &       & 79.92 & 76.64 \\
      & $[76.55;76.92]$ & $[77.61;79.84]$ &       & $[77.64;78.92]$ & $[77.73;78.72]$ &       & $[79.78;80.13]$ & $[76.45;77.03]$ \\
      &       &       &       &       &       &       &       &  \\
\multicolumn{1}{l}{\textit{Countries Liberalized in 1987-1991}} &       &       &       &       &       &       &       &  \\
\multirow{2}[0]{*}{$\tau_{\mathcal{Q}_2 k}$, Figure 5(c)} & 84.86 & 84.76 &       & 85.74 & 86.28 &       & 85.51 & 85.12 \\
      & $[84.47;85.30]$ & $[84.41;84.94]$ &       & $[85.45;86.44]$ & $[86.08;86.54]$ &       & $[84.86;85.92]$ & $[84.98;85.23]$ \\
      &       &       &       &       &       &       &       &  \\
\multicolumn{1}{l}{\textit{Countries Liberalized After 1991}} &       &       &       &       &       &       &       &  \\
\multirow{2}[1]{*}{$\tau_{\mathcal{Q}_3 k}$, Figure 5(e)} & 76.65 & 78.91 &       & 78.04 & 78.04 &       & 79.92 & 76.64 \\
      & $[76.55;76.92]$ & $[77.61;79.84]$ &       & $[77.64;78.92]$ & $[77.73;78.72]$ &       & $[79.78;80.13]$ & $[76.45;77.03]$ \\
\bottomrule
\bottomrule
\end{tabular}%


